Towards Online Steering of Flame Spray Pyrolysis Nanoparticle Synthesis

Flame Spray Pyrolysis (FSP) is a manufacturing technique to mass produce engineered nanoparticles for applications in catalysis, energy materials, composites, and more. FSP instruments are highly dependent on a number of adjustable parameters, including fuel injection rate, fuel-oxygen mixtures, and temperature, which can greatly affect the quality, quantity, and properties of the yielded nanoparticles. Optimizing FSP synthesis requires monitoring, analyzing, characterizing, and modifying experimental conditions.Here, we propose a hybrid CPU-GPU Difference of Gaussians (DoG)method for characterizing the volume distribution of unburnt solution, so as to enable near-real-time optimization and steering of FSP experiments. Comparisons against standard implementations show our method to be an order of magnitude more efficient. This surrogate signal can be deployed as a component of an online end-to-end pipeline that maximizes the synthesis yield.

==> figures/dog/dog.tex <==
\begin{figure*}[!htbp]
    \centering
    \definecolor{snowymint}{HTML}{E3F8D1}
    \definecolor{wepeep}{HTML}{FAD2D2}
    \definecolor{portafino}{HTML}{F5EE9D}
    \definecolor{plum}{HTML}{DCACEF}
    \definecolor{sail}{HTML}{A3CEEE}
    \definecolor{highland}{HTML}{6D885A}

    \tikzset{
        pics/filtersquare/.style args={#1/#2/#3/#4/#5}{
            code = {
                \draw[fill=#5] (#1,#2) rectangle (#3,#4);
                \draw[black, thick] (#1,#2) grid (#3,#4);
                \node at (#1+0.5,#2+0.5) {};
                \node at (#1+0.5,#2+1.5) {};
                \node at (#1+0.5,#2+2.5) {};
                \node at (#1+1.5,#2+0.5) {};
                \node at (#1+1.5,#2+1.5) {};
                \node at (#1+1.5,#2+2.5) {};
                \node at (#1+2.5,#2+0.5) {};
                \node at (#1+2.5,#2+1.5) {};
                \node at (#1+2.5,#2+2.5) {};
            }},
    }
    \begin{adjustbox}{width=\textwidth,center}

    \begin{tikzpicture}
        \tikzstyle{diff} = [draw, circle, scale=0.5]
        \node[yshift=-280, xshift=-400, inner sep=5pt] (bertrand) {\includegraphics[width=.35\textwidth]{figures/dog/bubbles.png}};

        \node[yshift=-280, xshift=-300, draw, circle, scale=1] (convol){\Large\(*\)};
        \draw[-] (bertrand) edge (convol);

        \foreach \Sigma in {0,...,5} {
            \node[yshift=-350+\Sigma*30,  xshift=-20, yslant=0.5, xslant=-1.5, scale=1] (bubbles-blur-\Sigma-1) {
                \includegraphics[width=.2\textwidth]{figures/dog/bubbles_sigma_\Sigma.png}
            };
        }

        \foreach \color/\Sigma in {snowymint/0, wepeep/1, portafino/2, plum/3, sail/4, highland/5} {
            \begin{scope}[
                every node/.append style={yslant=0.5, xslant=-1.5, opacity=.7, scale=.5},
                yshift=-370+\Sigma*30,
                xshift=-200,
                yslant=0.5,
                xslant=-1.5,
            ]
                \pic {filtersquare=0/0/3/3/\color};
                \coordinate (TL) at (0,1.5);
                \coordinate (BR) at (1.5, 0);
            \end{scope}
            \draw[-] (convol) edge (TL);
            \draw[-] (BR) edge (bubbles-blur-\Sigma-1);
        }

        \foreach \Sigma in {1,...,5} {
            \begin{scope}[
                yshift=-365+\Sigma*30, xshift=280,every node/.append style={
                    yslant=0.5, xslant=-1.5},yslant=0.5, xslant=-1.5
            ]
                \node[] (bubbles-dog-\Sigma-1) {
                    \includegraphics[width=.15\textwidth]{figures/dog/dog_bubbles_sigma_\Sigma.png}
                };
                \ifnum \Sigma>2
                \foreach \x in {-.8,-.6,-.4}  {
                    \foreach \y in {-.8,-.6,-.4} {
                        \fill[red!50] (\x,\y) rectangle (\x+.2,\y+.2);
                    }
                }
                \fi;

            \end{scope}

            \ifnum \Sigma>2 {
                \draw[yshift=-365+\Sigma*30, step=2mm, xshift=280, black, yslant=0.5, xslant=-1.5, opacity=0.3] (-1,-1) grid (0,0);
                \draw[yshift=-365+\Sigma*30, xshift=280, black, yslant=0.5, xslant=-1.5, opacity=0.3] (-1,-1) rectangle (0,0);
            }
            \fi;
            \ifnum \Sigma=4
            \fill[green, yshift=-365+\Sigma*30, xshift=280, yslant=0.5, xslant=-1.5, opacity=0.3] (-.6,-.6) rectangle (-.4,-.4)
            \fi;
        }

        \foreach \Sigma in {1,...,5} {
            \node[yshift=-365+\Sigma*30, xshift=140, diff] (diff-\Sigma-1){\Large\(-\)};
            \node[yshift=-365+\Sigma*30, xshift=160, diff] (plus-\Sigma-1){\Large\(\sigma_\Sigma\)};

        }


        % draw annotations
        \foreach \x in {1} {
            \foreach \Sigma in {1,...,5} {
                \draw[-] (bubbles-blur-\Sigma-\x) edge (diff-\Sigma-\x);
            }
            \foreach \Sigma in {0,...,4} {
                \pgfmathtruncatemacro{\nodelabel}{1+\Sigma}
                \draw[-] (bubbles-blur-\Sigma-\x) edge (diff-\nodelabel-\x);
            }
            \foreach \Sigma in {1,...,5} {
                \draw[-] (diff-\Sigma-\x) edge (plus-\Sigma-\x);
                \draw[->] (plus-\Sigma-\x) edge (bubbles-dog-\Sigma-\x);
            }
        }
    \end{tikzpicture}
    \end{adjustbox}
    \caption{Difference of Gaussians implemented as convolution by Gaussian kernels with $\mathtt{n\_bins} = 5$.}
    \label{fig:dogconv}
\end{figure*}

==> figures/doggpu.tex <==
\begin{figure}
        % Architecture
        \def\layerwidth{100pt}
        \def\layerheight{20pt}
        
        \tikzstyle{layer}=[style=block, draw, fill=black!20!white,
            inner sep=5pt,outer sep=0,
            text centered, 
            minimum width=2*\layerwidth, minimum height=\layerheight]
        \tikzstyle{block}=[draw=black,line width=1.0pt]
        
        \tikzstyle{fc}=[style=layer, fill=blue!30!white]
        \tikzstyle{conv}=[style=layer, fill=green!30!white]
        \tikzstyle{activation}=[style=layer, fill=orange!30!white]
        \tikzstyle{pool}=[style=layer, fill=red!30!white]
        \tikzstyle{bn}=[style=layer, fill=cyan!30!white]
        \tikzstyle{recurrent}=[style=layer, fill=purple!30!white]
        \tikzstyle{softmax}=[style=layer, fill=yellow!30!white]
        \tikzstyle{signal}=[arrows={-latex},draw=black,line width=1.5pt,rounded corners=4pt]
        \tikzstyle{point}=[]
        \centering
        \begin{tikzpicture}[
            start chain=going below, node distance=12pt,
            point/.append style={on chain, join=by {signal}},
            layer/.append style={on chain, join=by {signal}},
        ]
        \node[point] {Image};
        \node[conv] {$(\mathtt{n\_bin}+1) \times \mathtt{max\_width} \times \mathtt{max\_width}-$Conv2D};
        \node[fc] {$(\mathtt{n\_bins}+1)$-Diff-Mult};
        \node[pool] {$3 \times 3 \times 3-$MaxPool3D};
        \node[bn] {Thresh};
        \node[layer, dashed] {Prune};
        \node[point] {Blobs};
    \end{tikzpicture}
    \caption[]{GPU-DoG architecture}\label{fig:gpudog}
\end{figure}

==> figures/max_filter/max_filter.tex <==
\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{.45\textwidth}
        \centering
       \includegraphics[width=.9\textwidth]{figures/max_filter/coins.png} 
        \caption{Sample image}
        \label{fig:scalespace-blobs}
    \end{subfigure}
    
    \vspace*{1.5em}
    
    \begin{subfigure}{.45\textwidth}
        \centering
       \includegraphics[width=.9\textwidth]{figures/max_filter/max_filter.png} 
        \caption{Maximum of the image in a $3 \times 3$ neighborhood of each pixel}
        \label{fig:scalespace-plots}
    \end{subfigure}
    
    \vspace*{1.5em}
    
    \begin{subfigure}{.45\textwidth}
        \centering
       \includegraphics[width=.9\textwidth]{figures/max_filter/peaks.png} 
        \caption{Pixels which are equal to the local maximum}
        \label{fig:scalespace-plots}
    \end{subfigure}
    \caption{Local maxima heuristic example.}
    \label{fig:maxfilter}
\end{figure}



==> figures/precision_recall.tex <==
\begin{figure}
    \centering
        \begin{adjustbox}{width=.8\linewidth,center}

\begin{tikzpicture}[trim axis left]
% \begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
xlabel={difference},
ylabel={\#},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.0560353535353536, xmax=0.0767424242424242,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0, ymax=100.8,
ytick style={color=black}
]
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0133333333333332,0) rectangle (axis cs:-0.0126470690706383,1);
\addlegendimage{ybar,ybar legend,draw=none,fill=color0,fill opacity=0.5};
\addlegendentry{$\text{CPU}_p - \text{GPU}_p$}

\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0126470690706383,0) rectangle (axis cs:-0.0119608048079434,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0119608048079434,0) rectangle (axis cs:-0.0112745405452486,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0112745405452486,0) rectangle (axis cs:-0.0105882762825537,1);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0105882762825537,0) rectangle (axis cs:-0.0099020120198588,1);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0099020120198588,0) rectangle (axis cs:-0.00921574775716392,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00921574775716391,0) rectangle (axis cs:-0.00852948349446903,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00852948349446904,0) rectangle (axis cs:-0.00784321923177416,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00784321923177416,0) rectangle (axis cs:-0.00715695496907928,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00715695496907928,0) rectangle (axis cs:-0.0064706907063844,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.0064706907063844,0) rectangle (axis cs:-0.00578442644368952,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00578442644368952,0) rectangle (axis cs:-0.00509816218099464,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00509816218099464,0) rectangle (axis cs:-0.00441189791829976,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00441189791829976,0) rectangle (axis cs:-0.00372563365560488,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00372563365560488,0) rectangle (axis cs:-0.00303936939291,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00303936939291,0) rectangle (axis cs:-0.00235310513021512,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00235310513021512,0) rectangle (axis cs:-0.00166684086752024,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.00166684086752024,0) rectangle (axis cs:-0.000980576604825355,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.000980576604825355,0) rectangle (axis cs:-0.000294312342130476,0);
\draw[draw=none,fill=color0,fill opacity=0.5] (axis cs:-0.000294312342130476,0) rectangle (axis cs:0.000391951920564404,96);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.05,0) rectangle (axis cs:-0.0487929292929293,1);
\addlegendimage{ybar,ybar legend,draw=none,fill=color1,fill opacity=0.5};
\addlegendentry{$\text{CPU}_r - \text{GPU}_r$}

\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0487929292929293,0) rectangle (axis cs:-0.0475858585858586,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0475858585858586,0) rectangle (axis cs:-0.0463787878787879,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0463787878787879,0) rectangle (axis cs:-0.0451717171717172,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0451717171717172,0) rectangle (axis cs:-0.0439646464646465,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0439646464646465,0) rectangle (axis cs:-0.0427575757575758,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0427575757575758,0) rectangle (axis cs:-0.0415505050505051,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0415505050505051,0) rectangle (axis cs:-0.0403434343434344,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0403434343434344,0) rectangle (axis cs:-0.0391363636363637,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0391363636363637,0) rectangle (axis cs:-0.037929292929293,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.037929292929293,0) rectangle (axis cs:-0.0367222222222223,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0367222222222223,0) rectangle (axis cs:-0.0355151515151516,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0355151515151516,0) rectangle (axis cs:-0.0343080808080808,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0343080808080808,0) rectangle (axis cs:-0.0331010101010101,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0331010101010101,0) rectangle (axis cs:-0.0318939393939394,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0318939393939394,0) rectangle (axis cs:-0.0306868686868687,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0306868686868687,0) rectangle (axis cs:-0.029479797979798,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.029479797979798,0) rectangle (axis cs:-0.0282727272727273,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0282727272727273,0) rectangle (axis cs:-0.0270656565656566,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0270656565656566,0) rectangle (axis cs:-0.0258585858585859,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0258585858585859,0) rectangle (axis cs:-0.0246515151515152,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0246515151515152,0) rectangle (axis cs:-0.0234444444444445,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0234444444444445,0) rectangle (axis cs:-0.0222373737373738,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0222373737373738,0) rectangle (axis cs:-0.0210303030303031,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0210303030303031,0) rectangle (axis cs:-0.0198232323232323,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0198232323232324,0) rectangle (axis cs:-0.0186161616161616,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0186161616161616,0) rectangle (axis cs:-0.0174090909090909,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0174090909090909,0) rectangle (axis cs:-0.0162020202020202,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0162020202020202,0) rectangle (axis cs:-0.0149949494949495,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0149949494949495,0) rectangle (axis cs:-0.0137878787878788,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0137878787878788,0) rectangle (axis cs:-0.0125808080808081,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0125808080808081,0) rectangle (axis cs:-0.0113737373737374,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0113737373737374,0) rectangle (axis cs:-0.0101666666666667,3);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.0101666666666667,0) rectangle (axis cs:-0.00895959595959598,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00895959595959598,0) rectangle (axis cs:-0.00775252525252527,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00775252525252527,0) rectangle (axis cs:-0.00654545454545456,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00654545454545456,0) rectangle (axis cs:-0.00533838383838386,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00533838383838386,0) rectangle (axis cs:-0.00413131313131315,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00413131313131315,0) rectangle (axis cs:-0.00292424242424244,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00292424242424244,0) rectangle (axis cs:-0.00171717171717174,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00171717171717174,0) rectangle (axis cs:-0.00051010101010103,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:-0.00051010101010103,0) rectangle (axis cs:0.000696969696969682,67);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.000696969696969682,0) rectangle (axis cs:0.00190404040404039,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00190404040404039,0) rectangle (axis cs:0.00311111111111109,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00311111111111109,0) rectangle (axis cs:0.0043181818181818,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0043181818181818,0) rectangle (axis cs:0.00552525252525251,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00552525252525251,0) rectangle (axis cs:0.00673232323232322,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00673232323232322,0) rectangle (axis cs:0.00793939393939393,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00793939393939393,0) rectangle (axis cs:0.00914646464646463,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.00914646464646463,0) rectangle (axis cs:0.0103535353535353,6);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0103535353535353,0) rectangle (axis cs:0.011560606060606,7);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.011560606060606,0) rectangle (axis cs:0.0127676767676768,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0127676767676768,0) rectangle (axis cs:0.0139747474747475,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0139747474747475,0) rectangle (axis cs:0.0151818181818182,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0151818181818182,0) rectangle (axis cs:0.0163888888888889,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0163888888888889,0) rectangle (axis cs:0.0175959595959596,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0175959595959596,0) rectangle (axis cs:0.0188030303030303,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0188030303030303,0) rectangle (axis cs:0.020010101010101,2);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.020010101010101,0) rectangle (axis cs:0.0212171717171717,2);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0212171717171717,0) rectangle (axis cs:0.0224242424242424,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0224242424242424,0) rectangle (axis cs:0.0236313131313131,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0236313131313131,0) rectangle (axis cs:0.0248383838383838,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0248383838383838,0) rectangle (axis cs:0.0260454545454545,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0260454545454545,0) rectangle (axis cs:0.0272525252525253,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0272525252525253,0) rectangle (axis cs:0.028459595959596,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.028459595959596,0) rectangle (axis cs:0.0296666666666667,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0296666666666667,0) rectangle (axis cs:0.0308737373737374,3);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0308737373737374,0) rectangle (axis cs:0.0320808080808081,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0320808080808081,0) rectangle (axis cs:0.0332878787878788,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0332878787878788,0) rectangle (axis cs:0.0344949494949495,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0344949494949495,0) rectangle (axis cs:0.0357020202020202,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0357020202020202,0) rectangle (axis cs:0.0369090909090909,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0369090909090909,0) rectangle (axis cs:0.0381161616161616,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0381161616161616,0) rectangle (axis cs:0.0393232323232323,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0393232323232323,0) rectangle (axis cs:0.040530303030303,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.040530303030303,0) rectangle (axis cs:0.0417373737373737,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0417373737373737,0) rectangle (axis cs:0.0429444444444445,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0429444444444445,0) rectangle (axis cs:0.0441515151515152,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0441515151515152,0) rectangle (axis cs:0.0453585858585859,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0453585858585859,0) rectangle (axis cs:0.0465656565656566,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0465656565656566,0) rectangle (axis cs:0.0477727272727273,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0477727272727273,0) rectangle (axis cs:0.048979797979798,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.048979797979798,0) rectangle (axis cs:0.0501868686868687,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0501868686868687,0) rectangle (axis cs:0.0513939393939394,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0513939393939394,0) rectangle (axis cs:0.0526010101010101,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0526010101010101,0) rectangle (axis cs:0.0538080808080808,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0538080808080808,0) rectangle (axis cs:0.0550151515151515,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0550151515151515,0) rectangle (axis cs:0.0562222222222222,1);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0562222222222222,0) rectangle (axis cs:0.0574292929292929,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0574292929292929,0) rectangle (axis cs:0.0586363636363637,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0586363636363637,0) rectangle (axis cs:0.0598434343434344,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0598434343434344,0) rectangle (axis cs:0.0610505050505051,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0610505050505051,0) rectangle (axis cs:0.0622575757575758,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0622575757575758,0) rectangle (axis cs:0.0634646464646465,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0634646464646465,0) rectangle (axis cs:0.0646717171717172,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0646717171717172,0) rectangle (axis cs:0.0658787878787879,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0658787878787879,0) rectangle (axis cs:0.0670858585858586,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0670858585858586,0) rectangle (axis cs:0.0682929292929293,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0682929292929293,0) rectangle (axis cs:0.0695,0);
\draw[draw=none,fill=color1,fill opacity=0.5] (axis cs:0.0695,0) rectangle (axis cs:0.0707070707070707,1);
\end{axis}


\end{tikzpicture}
\end{adjustbox}

    \caption{Distribution of precision $\text{CPU}_p - \text{GPU}_p$ and recall $\text{CPU}_r - \text{GPU}_r$ difference pairs for 100 simulated samples.}
    \label{fig:precisionrecall}
\end{figure}
